HiT-SR: Hierarchical Transformer for Efficient Image Super-Resolution

Transformers have exhibited promising performance in computer vision tasks including image super-resolution (SR). However, popular transformer-based SR methods often employ window self-attention with quadratic computational complexity to window sizes, resulting in fixed small windows with limited receptive fields. In this paper, we present a general strategy to convert transformer-based SR networks to hierarchical transformers (HiT-SR), boosting SR performance with multi-scale features while maintaining an efficient design. Specifically, we first replace the commonly used fixed small windows with expanding hierarchical windows to aggregate features at different scales and establish long-range dependencies. Considering the intensive computation required for large windows, we further design a spatial-channel correlation method with linear complexity to window sizes, efficiently gathering spatial and channel information from hierarchical windows. Extensive experiments verify the effectiveness and efficiency of our HiT-SR, and our improved versions of SwinIR-Light, SwinIR-NG, and SRFormer-Light yield state-of-the-art SR results with fewer parameters, FLOPs, and faster speeds ($\sim7\times$).

==> tabs/main/tab-main-backup.tex <==
\begin{table*}[!ht]
\scriptsize
\begin{center}
\begin{tabular}{l|c|cc|ccccccccccccccc} 
\toprule[0.15em]
	\rowcolor{color3}  &  & \multicolumn{2}{c|}{Complexity} & \multicolumn{2}{c}{Set5} & \multicolumn{2}{c}{Set14} & \multicolumn{2}{c}{B100} & \multicolumn{2}{c}{Urban100} & \multicolumn{2}{c}{Manga109}\\

	\rowcolor{color3} \multirow{-2}{*}{Method}& \multirow{-2}{*}{Scale} & \#Para. & FLOPs & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM
\\
\midrule[0.15em]
EDSR-baseline \cite{lim2017edsr} & $\times$2 & 1370K & 316.3G &
37.99 & 0.9604 & 33.57 & 0.9175 & 32.16 & 0.8994 & 31.98 & 0.9272 & 38.54 & 0.9769\\
CARN \cite{ahn2018carn} & $\times$2 & 1592K & 222.8G &
37.76 & 0.9590 & 33.52 & 0.9166 & 32.09 & 0.8978 & 31.92 & 0.9256 & 38.36 & 0.9765\\
IMDN \cite{hui2019imdn} & $\times$2 & 694K & 158.8G &
38.00 & 0.9605 & 33.63 & 0.9177 & 32.19 & 0.8996 & 32.17 & 0.9283 & 38.88 & 0.9774\\
LatticeNet \cite{luo2020latticenet} & $\times$2 & 756K & 169.5G &
38.06  & 0.9607 & 33.70 & 0.9187 & 32.20 & 0.8999 & 32.25 & 0.9288 & 38.94 & 0.9774\\
RFDN-L \cite{liu2020rfdn} & $\times$2 & 626K & 145.8G &
38.08 & 0.9606 & 33.67 & 0.9190 & 32.18 & 0.8996 & 32.24 & 0.9290 & 38.95 & 0.9773\\
SRPN-Lite \cite{zhang2021srpn} & $\times$2 & 609K & 139.9G &
38.10 & 0.9608 & 33.70 & 0.9189 & 32.25 & 0.9005 & 32.26 & 0.9294 & - & -\\
FMEN \cite{du2022fmen} & $\times$2 & 748K & 172.0G &
38.10 & 0.9609 & 33.75 & 0.9192 & 32.26 & 0.9007 & 32.41 & 0.9311 & 38.95 & 0.9778\\
GASSL-B \cite{wang2023gassl} & $\times$2 & 689K & 158.2G &
38.08 & 0.9607 & 33.75 & 0.9194 & 32.24 & 0.9005 & 32.29 & 0.9298 & 38.92 & 0.9777\\
SwinIR-Light \cite{liang2021swinir} & $\times$2 & 910K & 244.4G &
38.14 & 0.9611 & 33.86 & 0.9206 & 32.31 & 0.9012 & 32.76 & 0.9340 & 39.12 & 0.9783\\
HNCT \cite{fang2022hnct} & $\times$2 & 357K & 82.4G &
38.08 & 0.9608 & 33.65 & 0.9182 & 32.22 & 0.9001 & 32.22 & 0.9294 & 38.87 & 0.9774\\
ELAN-Light \cite{zhang2022elan} & $\times$2 & 621K & 201.3G &
\textcolor{blue}{38.17} & 0.9611 & 33.94 & 0.9207 & 32.30 & 0.9012 & 32.76 & 0.9340 & 39.11 & 0.9782\\
SwinIR-NG \cite{choi2023ngram} & $\times$2 & 1181K & 274.1G &
\textcolor{blue}{38.17} & \textcolor{blue}{0.9612} & 33.94 & 0.9205 & 32.31 & 0.9013 & 32.78 & 0.9340 & 39.20 & 0.9781\\
% DAT-Light \cite{choi2023ngram} & $\times$2 & 553K & 194.26G &
% 38.24 & 0.9614 & 34.01 & 0.9214 & 32.34 & 0.9019 & 32.89 & 0.9346 & 39.49 & 0.9788\\
\textbf{HiT-SIR-S (Ours)} & $\times$2 & 495K & 137.4G & 38.16
 & 0.9611 & 33.83 & 0.9202 & 32.29 & 0.9013 & 32.79 & 0.9343 & 39.32 & 0.9785\\
\textbf{HiT-SIR (Ours)} & $\times$2 & 772K & 209.9G & \textcolor{red}{38.23}
 & \textcolor{blue}{0.9612} & \textcolor{blue}{33.96} & \textcolor{blue}{0.9212} & \textcolor{blue}{32.35} & \textcolor{blue}{0.9020} & \textcolor{blue}{33.02} & \textcolor{blue}{0.9363} & \textcolor{blue}{39.50} & \textcolor{blue}{0.9788}\\
\textbf{HiT-SNG (Ours)} & $\times$2 & \textcolor{black}{1013K} & \textcolor{black}{213.9G}  & \textcolor{red}{38.23}
 & \textcolor{red}{0.9613} & \textcolor{red}{33.98} & \textcolor{red}{0.9217} & \textcolor{red}{32.36} & \textcolor{red}{0.9021} & \textcolor{red}{33.06} & \textcolor{red}{0.9366} & \textcolor{red}{39.51} & \textcolor{red}{0.9789}\\
% \textbf{HiT-DAT (Ours)} & $\times$2 &  &  &
%  &  &  &  &  &  &  &  &  & \\

% SwinIR & $\times$2 & & & 
% {38.42} & {0.9623} & {34.46} & {0.9250} &{32.53} &{0.9041} & {33.81} &{0.9427} & {39.92} & {0.9797}\\
% CAT-A & $\times$2 & & & 
% \textcolor{black}{38.51} & \textcolor{black}{0.9626} & \textcolor{black}{34.78} & \textcolor{black}{0.9265} & \textcolor{black}{32.59} & \textcolor{black}{0.9047} & \textcolor{black}{34.26} & \textcolor{black}{0.9440} & \textcolor{black}{40.10} & \textcolor{black}{0.9805}
% \\ 
% DAT-S (ours) & $\times$2 &  & &
% \textcolor{black}{38.54} & \textcolor{black}{0.9627} & \textcolor{black}{34.60} & \textcolor{black}{0.9258} & \textcolor{black}{32.57} & \textcolor{black}{0.9047} & \textcolor{black}{34.12} & \textcolor{black}{0.9444} & \textcolor{black}{40.17} & \textcolor{black}{0.9804}
% \\ 
% DAT (ours) & $\times$2 &  & &
% \textcolor{blue}{38.58} & \textcolor{blue}{0.9629} & \textcolor{blue}{34.81} & \textcolor{blue}{0.9272} & \textcolor{blue}{32.61} & \textcolor{blue}{0.9051} & \textcolor{blue}{34.37} & \textcolor{blue}{0.9458} & \textcolor{blue}{40.33} & \textcolor{blue}{0.9807}
% \\ 
% DAT+ (ours) & $\times$2 &  & &
% \textcolor{red}{38.63} & \textcolor{red}{0.9631} & \textcolor{red}{34.86} & \textcolor{red}{0.9274} & \textcolor{red}{32.63} & \textcolor{red}{0.9053} & \textcolor{red}{34.47} & \textcolor{red}{0.9465} & \textcolor{red}{40.43} & \textcolor{red}{0.9809}
% \\

%% x3 scale ======================================
\midrule
EDSR-baseline \cite{lim2017edsr} & $\times$3 & 1555K & 160.2G &
34.37 & 0.9270 & 30.28  & 0.8417 & 29.09 & 0.8052 & 28.15 & 0.8527 & 33.45 & 0.9439\\
CARN \cite{ahn2018carn} & $\times$3 & 1592K & 118.8G &
34.29 & 0.9255 & 30.29 & 0.8407 & 29.06 & 0.8034 & 28.06 & 0.8493 & 33.50 & 0.9440\\
IMDN \cite{hui2019imdn} & $\times$3 & 703K & 71.5G &
34.36 & 0.9270 & 30.32 & 0.8417 & 29.09 & 0.8046 & 28.17 & 0.8519 & 33.61 & 0.9445\\
LatticeNet \cite{luo2020latticenet} & $\times$3 & 765K & 76.3G &
34.40  & 0.9272 & 30.32 & 0.8416 & 29.10 & 0.8049 & 28.19 & 0.8513 & 33.63 & 0.9442\\
RFDN-L \cite{liu2020rfdn} & $\times$3 & 633K & 65.6G &
34.47 & 0.9280 & 30.35 & 0.8421 & 29.11 & 0.8053 & 28.32 & 0.8547 & 33.78 & 0.9458\\
SRPN-Lite \cite{zhang2021srpn} & $\times$3 & 615K & 62.7G &
34.47 & 0.9276 & 30.38 & 0.8425 & 29.16 & 0.8061 & 28.22 & 0.8534 & - & -\\
FMEN \cite{du2022fmen} & $\times$3 & 757K & 77.2G &
34.45 & 0.9275 & 30.40 & 0.8435 & 29.17 & 0.8063 & 28.33 & 0.8562 & 33.86 & 0.9462\\
GASSL-B \cite{wang2023gassl} & $\times$3 & 691K & 70.4G &
34.47 & 0.9278 & 30.39 & 0.8430 & 29.15 & 0.8063 & 28.27 & 0.8546 & 33.77 & 0.9455\\
SwinIR-Light \cite{liang2021swinir} & $\times$3 & 918K & 110.8G &
34.62 & 0.9289 & 30.54 & 0.8463 & 29.20 & 0.8082 & 28.66 & 0.8624 & 33.98 & 0.9478\\
HNCT \cite{fang2022hnct} & $\times$3 & 363K & 37.8G &
34.47 & 0.9275 & 30.44 & 0.8439 & 29.15 & 0.8067 & 28.28 & 0.8557 & 33.81 & 0.9459\\
ELAN-Light \cite{zhang2022elan} & $\times$3 & 629K & 89.5G &
34.61 & 0.9288 & 30.55 & 0.8463 & 29.21 & 0.8081 & 28.69 & 0.8624 & 34.00 & 0.9478\\
SwinIR-NG \cite{choi2023ngram} & $\times$3 & 1190K & 114.1G &
34.64 & 0.9293 & \textcolor{black}{30.58} & 0.8471 & \textcolor{blue}{29.24} & \textcolor{blue}{0.8090} & 28.75 & 0.8639 & 34.22 & 0.9488\\
% DAT-Light \cite{choi2023ngram} & $\times$3 & 561K & 88.59G &
% 34.76 & 0.9299 & 30.63 & 0.8474 & 29.29 & 0.8103 & 28.89 & 0.8666 & 34.55 & 0.9501\\
\textbf{HiT-SIR-S (Ours)} & $\times$3 & 501K & 61.8G & 34.62
 & 0.9289 & 30.54 & 0.8460 & 29.22 & 0.8087 & \textcolor{blue}{28.79} & \textcolor{blue}{0.8644} & \textcolor{blue}{34.33} & 0.9488\\
\textbf{HiT-SIR (Ours)} & $\times$3 & 780K & 94.2G & \textcolor{blue}{34.72}
 & \textcolor{blue}{0.9297} & \textcolor{red}{30.65} & \textcolor{blue}{0.8477} & \textcolor{red}{29.28} & \textcolor{red}{0.8102} & \textcolor{red}{28.99} & \textcolor{red}{0.8687} & \textcolor{red}{34.56} & \textcolor{blue}{0.9501} \\
\textbf{HiT-SNG (Ours)} & $\times$3 & \textcolor{black}{1021K} & \textcolor{black}{99.5G} & \textcolor{red}{34.74}
 & \textcolor{red}{0.9298} & \textcolor{blue}{30.64} & \textcolor{red}{0.8479} & \textcolor{red}{29.28} & \textcolor{red}{0.8102} & \textcolor{red}{28.99} & \textcolor{red}{0.8687} & \textcolor{red}{34.56} & \textcolor{red}{0.9502} \\
 
%% x4 scale ======================================
\midrule
EDSR-baseline \cite{lim2017edsr} & $\times$4 & 1518K & 114.0G &
32.09 & 0.8938 & 28.58 & 0.7813 & 27.57 & 0.7357 & 26.04 & 0.7849 & 30.35 & 0.9067\\
CARN \cite{ahn2018carn} & $\times$4 & 1592K & 90.9G &
32.13 & 0.8937 & 28.60 & 0.7806 & 27.58 & 0.7349 & 26.07 & 0.7837 & 30.47 & 0.9084\\
IMDN \cite{hui2019imdn} & $\times$4 & 715K & 40.9G &
32.21 & 0.8948 & 28.58 & 0.7811 & 27.56 & 0.7353 & 26.04 & 0.7838 & 30.45 & 0.9075\\
LatticeNet \cite{luo2020latticenet} & $\times$4 & 777K & 43.6G &
32.18  & 0.8943 & 28.61 & 0.7812 & 27.57 & 0.7355 & 26.14 & 0.7844 & 30.54 & 0.9075\\
RFDN-L \cite{liu2020rfdn} & $\times$4 & 643K & 37.4G &
32.28 & 0.8957 & 28.61 & 0.7818 & 27.58 & 0.7363 & 26.20 & 0.7883 & 30.61 & 0.9096\\
SRPN-Lite \cite{zhang2021srpn} & $\times$4 & 623K & 35.8G &
32.24 & 0.8958 & 28.69 & 0.7836 & 27.63 & 0.7373 & 26.16 & 0.7875 & - & -\\
FMEN \cite{du2022fmen} & $\times$4 & 769K & 44.2G &
32.24 & 0.8955 & 28.70 & 0.7839 & 27.63 & 0.7379 & 26.28 & 0.7908 & 30.70 & 0.9107\\
GASSL-B \cite{wang2023gassl} & $\times$4 & 694K & 39.9G &
32.17 & 0.8950 & 28.66 & 0.7835 & 27.62 & 0.7377 & 36.16 & 0.7888 & 30.70 & 0.9100\\
SwinIR-Light \cite{liang2021swinir} & $\times$4 & 930K & 63.6G &
32.44 & 0.8976 & 28.77 & 0.7858 & 27.69 & 0.7406 & 26.47 & 0.7980 & 30.92 & 0.9151\\
HNCT \cite{fang2022hnct} & $\times$4 & 373K & 22.0G &
32.31 & 0.8957 & 28.71 & 0.7834 & 27.63 & 0.7381 & 26.20 & 0.7896 & 30.70 & 0.9112\\
ELAN-Light \cite{zhang2022elan} & $\times$4 & 640K & 53.7G &
32.43 & 0.8975 & 28.78 & 0.7858 & 27.69 & 0.7406 & 26.54 & 0.7982 & 30.92 & 0.9150\\
SwinIR-NG \cite{choi2023ngram} & $\times$4 & 1201K & 64.4G &
32.44 & 0.8980 & \textcolor{blue}{28.83} & \textcolor{blue}{0.7870} & \textcolor{blue}{27.73} & \textcolor{blue}{0.7418} & 26.61 & 0.8010 & 31.09 & 0.9161\\
% DAT-Light \cite{choi2023ngram} & $\times$4 & 573K & 49.69G &
% 32.57 & 0.8991 & 28.87 & 0.7879 & 27.74 & 0.7428 & 26.64 & 0.8033 & 31.37 & 0.9178\\
\textbf{HiT-SIR-S (Ours)} & $\times$4 & 511K & 35.4G & 32.44
& 0.8978 & 28.82 & 0.7866 & 27.68 & 0.7409 & 26.61 & 0.8013  & 31.11 & 0.9151 \\
\textbf{HiT-SIR (Ours)} & $\times$4 & 792K & 53.8G & \textcolor{blue}{32.54}
 & \textcolor{blue}{0.8994} & \textcolor{red}{28.90} & \textcolor{red}{0.7882} & \textcolor{blue}{27.73} & \textcolor{red}{0.7429} & \textcolor{blue}{26.83} & \textcolor{blue}{0.8072} & \textcolor{blue}{31.37} & \textcolor{blue}{0.9177} \\
\textbf{HiT-SNG (Ours)} & $\times$4 & \textcolor{black}{1032K} & \textcolor{black}{57.7G} & \textcolor{red}{32.55}
 & \textcolor{red}{0.8995} & \textcolor{red}{28.90} & \textcolor{red}{0.7882} & \textcolor{red}{27.74} & \textcolor{red}{0.7429} & \textcolor{red}{26.85} & \textcolor{red}{0.8076} & \textcolor{red}{31.38} & \textcolor{red}{0.9180} \\
\bottomrule[0.15em]
\end{tabular}
\vspace{-1mm}
\caption{Quantitative comparison with state-of-the-art efficient SR methods, where HiT-SIR-S indicates HiT-SIR with reduced dimension. The best and second-best SR results are colored \textcolor{red}{red} and \textcolor{blue}{blue}. The output size is set to $3\times 720 \times 1280$ for all scales to compute FLOPs. 
% \textcolor{red}{(modify the complexity of HiT-SNG)}
}
\label{table:quantires}
\end{center}
% \vspace{-8mm}
\vspace{-2.8em}
\end{table*}
